Orthus: Autoregressive Interleaved Image-Text Generation with Modality-Specific Heads

We introduce Orthus, an autoregressive (AR) transformer that excels in generating images given textual prompts, answering questions based on visual inputs, and even crafting lengthy image-text interleaved contents. Unlike prior arts on unified multimodal modeling, Orthus simultaneously copes with discrete text tokens and continuous image features under the AR modeling principle. The continuous treatment of visual signals minimizes the information loss for both image understanding and generation while the fully AR formulation renders the characterization of the correlation between modalities straightforward. The key mechanism enabling Orthus to leverage these advantages lies in its modality-specific heads -- one regular language modeling (LM) head predicts discrete text tokens and one diffusion head generates continuous image features conditioning on the output of the backbone. We devise an efficient strategy for building Orthus -- by substituting the Vector Quantization (VQ) operation in the existing unified AR model with a soft alternative, introducing a diffusion head, and tuning the added modules to reconstruct images, we can create an Orthus-base model effortlessly (e.g., within mere 72 A100 GPU hours). Orthus-base can further embrace post-training to better model interleaved images and texts. Empirically, Orthus surpasses competing baselines including Show-o and Chameleon across standard benchmarks, achieving a GenEval score of 0.58 and an MME-P score of 1265.8 using 7B parameters. Orthus also shows exceptional mixed-modality generation capabilities, reflecting the potential for handling intricate practical generation tasks.

==> sec/0_abstract_arxiv.tex <==
% \vspace{-4pt}
\begin{abstract}
We introduce Orthus, an autoregressive (AR) transformer that excels in generating images given textual prompts, answering questions based on visual inputs, and even crafting lengthy image-text interleaved contents. 
Unlike prior arts on unified multimodal modeling, Orthus simultaneously copes with \textbf{discrete text tokens} and \textbf{continuous image features} under the \textbf{AR} modeling principle.
% transformer backbone with two dedicated heads for text and image decoding. 
The continuous treatment of visual signals minimizes the information loss for both image understanding and generation while the fully AR formulation renders the characterization of the correlation between modalities straightforward. 
The key mechanism enabling Orthus to leverage these advantages lies in its modality-specific heads---one regular language modeling (LM) head predicts discrete text tokens and one diffusion head generates continuous image features conditioning on the output of the backbone. 
% In practice, Orthus operates on the hidden representation of a pre-trained image variational autoencoder (VAE) for state compression. 
% Unlike fully token-based autoregressive (AR) models, Orthus adopts continuous image representations from a VAE encoder, avoiding information loss caused by Vector Quantization (VQ). 
% Compared with prior studies that unify autoregressive and diffusion in a single transformer, Orthus is pure AR by disentangling diffusion from the backbone, making it more suited to image-text interleaved modeling (because the backbone does not need to accept noisy images during training). 
We devise an efficient strategy for building Orthus---by substituting the Vector Quantization (VQ) operation in the existing unified AR model with a soft alternative, introducing a diffusion head, and tuning the added modules to reconstruct images, we can create an Orthus-base model effortlessly (e.g., within mere 72 A100 GPU hours). 
Orthus-base can further embrace post-training to better model interleaved images and texts. 
Empirically, Orthus surpasses competing baselines including Show-o and Chameleon across standard benchmarks, achieving a GenEval score of 0.58 and an MME-P score of 1265.8 using 7B parameters. %, outperforming specialized text-to-image models like SDXL.
Orthus also shows exceptional mixed-modality generation capabilities, reflecting the potential for handling intricate practical generation tasks.
% Our code is available at \small{\url{https://github.com/zhijie-group/Orthus}}.
\end{abstract}

 % bypasses the need to add noise (whether [mask] tokens or Gaussian noise) to the image before processing it in the transformer, enabling more effective multimodal learning.
 % Specifically, Orthus accepts discrete text tokens and continuous image features as inputs and is composed of a unified transformer backbone and two dedicated heads for text and image decoding respectively. The backbone auto-regressively models the correlation, while the heads yield discrete text tokens and continuous image features, respectively. The heads are trained under typical softmax cross-entropy and diffusion modeling rules. Unlike fully autoregressive (AR) models, Orthus adopts continuous, lossless patch-wise image features from a VAE encoder and enjoys enhanced image-generation quality benefits from Vector Quantization (VQ)-free representations.

==> tabs/geneval.tex <==
\begin{table*}[h]
    \centering
    \caption{\textbf{Comparison with state-of-the-arts on visual generation benchmarks.} Und. and Gen. denote ``understanding'' and ``generation'', respectively. Model using external pre-trained diffusion model is marked with * and $\text{Chameleon}^\dagger$ is post-trained with the same dataset as Orthus. The results in \textbf{bold} and \underline{underline} are the best and second-best results, respectively.} 
    \setlength{\tabcolsep}{3.6pt}
    \scalebox{0.9}{
    \begin{tabular}{clccccccccc}
        \hline
        \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Res.}} & \multicolumn{7}{c}{\textbf{GenEval} $\uparrow$ }                                       & \multirow{2}{*}{\textbf{HPSv2}$\uparrow$} \\ \cline{4-10}
                              &                        &                         & Single Obj. & Two Obj. & Count. & Colors & Position & Color Attri. & Overall &                      \\ \hline

        % \midrule
        \multirow{6}{*}{\shortstack{Gen. \\ Only}} 
        
        % & LlamaGen~\cite{sun2024autoregressive}  & 512 & 0.71 & 0.34 & 0.21 & 0.58 & 0.07 & 0.04 & 0.32 & 26.3 \\
        & SDv1.5~\cite{rombach2022high} & 512 & 0.97 & 0.38 & 0.35 & 0.76 & 0.04 & 0.06 & 0.43 & 27.0 \\
        % & PixArt-$\alpha$~\cite{chen2024pixartalpha} & 512 & 0.98 & 0.50 & 0.44 & 0.80 & 0.08 & 0.07 & 0.48 & - \\
        & SDv2.1~\cite{rombach2022high} & 512 & 0.98 & 0.51 & 0.44 & 0.85 & 0.07 & 0.17 & 0.50 & 27.2 \\
        & DALL-E 2~\cite{ramesh2022hierarchical} & 512 & 0.94 & 0.66 & 0.49 & 0.77 & 0.10 & 0.19 & 0.52 & 26.9 \\
        & Emu3-Gen~\cite{wang2024emu3} & 512 & 0.98 & 0.71 & 0.34 & 0.81 & 0.17 & 0.21 & 0.54 & - \\
        & SDXL~\cite{podellsdxl} & 512 & 0.98 & 0.74 & 0.39 & 0.85 & 0.15 & 0.23 & 0.55 & 30.9 \\
        & SD3(d=30)~\cite{esser2024scaling} & 512 & 0.96 & 0.80 & 0.65 & 0.73 & 0.33 & 0.37 & 0.64 & - \\
        \midrule
        \multirow{7}{*}{\shortstack{Und. \\ \& \\ Gen.}} & $\text{SEED-X}^{*}$~\cite{ge2024seed} & 448 & 0.97 & 0.58 & 0.26 & 0.80 & 0.19 & 0.14 & 0.49 & - \\
        & Chameleon~\cite{team2024chameleon} & 512 & - & - & - & - & - & - & 0.39 & - \\
        & LWM~\cite{liu2024world} & 256 & 0.93 & 0.41 & 0.46 & 0.79 & 0.09 & 0.15 & 0.47 & 26.1 \\
        & Show-o~\cite{xie2024show} & 256 & 0.95 & 0.52 & \textbf{0.49} & 0.82 & 0.11 & 0.28 & 0.53 & 27.3 \\
        & Transfusion~\cite{zhou2024transfusion} & 256 & - & - & - & - & - & - & \textbf{0.63} & - \\
        & $\text{Chameleon}^{\dagger}$ & 512 & 0.98 & 0.47 & 0.18 & 0.75 & 0.06 & 0.15 & 0.43 & 26.9 \\
        & \textbf{Orthus (Ours)} & 512 & \textbf{0.99} & \textbf{0.75} & 0.26 & \textbf{0.84} & \textbf{0.28} & \textbf{0.38} & \underline{0.58} & \textbf{28.2} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:geneval}
\end{table*}

==> tabs/hps.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison of state-of-art baselines on HPSv2.}
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Model}  & Ani. & Conc. & Paint. & Pho. & \textbf{Overall}$\uparrow$ \\
    \midrule
    LDM~\cite{rombach2022high} & 25.7 & 25.2 & 25.3 & 27.0 & 25.8 \\
    DALL-E 2~\cite{ramesh2022hierarchical} & 27.3 & 26.5 & 26.7 & 27.2 & 26.9 \\ 
    SDv1.5~\cite{rombach2022high} & 27.3 & 26.6 & 26.7 & 27.3 & 27.0 \\
    SDv2~\cite{rombach2022high} & 27.5 & 26.9 & 26.9 & 27.5 & 27.2 \\
    SDXL~\cite{podellsdxl} & 36.0 & 34.9 & 35.7 & 31.9 & 30.9 \\
    Show-o~\cite{xie2024show} & 27.9 & 27.3 & 27.1 & 27.0 & 27.3 \\
    $\text{Chameleon}^{\dagger}$ & 26.9 & 27.2 & 27.3 & 26.0 & 26.9 \\
    \textbf{Orthus(Ours)} & 28.2 & 28.4 & 28.4 & 27.8 & 28.2 \\
    \bottomrule
    \end{tabular}
    \label{tab:hps}
    \vspace{-14pt}
\end{table}
